On the Convergence of Bounded Agents

When has an agent converged? Standard models of the reinforcement learning problem give rise to a straightforward definition of convergence: An agent converges when its behavior or performance in each environment state stops changing. However, as we shift the focus of our learning problem from the environment's state to the agent's state, the concept of an agent's convergence becomes significantly less clear. In this paper, we propose two complementary accounts of agent convergence in a framing of the reinforcement learning problem that centers around bounded agents. The first view says that a bounded agent has converged when the minimal number of states needed to describe the agent's future behavior cannot decrease. The second view says that a bounded agent has converged just when the agent's performance only changes if the agent's internal state changes. We establish basic properties of these two definitions, show that they accommodate typical views of convergence in standard settings, and prove several facts about their nature and relationship. We take these perspectives, definitions, and analysis to bring clarity to a central idea of the field.

==> proofs/thm-pconv_mdp_qlearning.tex <==
\begin{dproof}[\cref{thm:pconv_mdp_qlearning}]

\textcolor{blue}{Note: Missing detail(s) about how boundedness impacts Q-learning.}

First, we clarify what is meant by ``the conditions required by the central Theorem of \citet{watkins1992q} hold of $\agent$ and $\environment$.'' Recall that a tabular Q-learning agent maintains a Q function for each environment-state and action pair. Since the environment is an MDP, we let the observation $o_t \in \observations$ denote the environment state at time $t$, and thus the function maintained by the agent is updated according to,
%\begin{multline*}
\[
Q_{t+1}(o_t,a_t) = Q_{t}(o_t, a_t) + \alpha_t \\
\left(r(o_t) + \gamma \max_{a' \in \actions} Q_{t}(o_{t+1},a')  - Q_{t}(o_{t+1}, a_t) \right),
\]
%\end{multline*}
for all time-steps $t \geq 0$.%We suppose $Q_0$ is initialized to be all zeros, but this .


Recall further that the conditions required by \citet{watkins1992q} of agent and environment to ensure convergence of the sequence of Q-values maintained by the agent:
\begin{enumerate}
    \item The step size $\alpha_t$, satisfies the Robbins-Monro conditions \cite{robbins1951stochastic}:
    \begin{equation}
        \sum_{t=0}^\infty \alpha_t = \infty, \hspace{8mm} \sum_{t=0}^\infty \alpha_t^2 < \infty.
    \end{equation}
    
    \item The environment is an MDP: $o_t \sim e(h_{t-1}, a_{t-1})$ can be expressed as simply $o_t \sim e(o_{t-1}, a_{t-1})$, and $r(h_t)$ can be expressed as $r(o_{t-1})$.%, where $\exists_{r_{\text{max}}}\ \max_{o \in \observations} r(o) \leq r_{\text{max}}$.
    
    \item Performance $\valuef$ is assessed according to expected discounted return with discount $\gamma \in [0,1)$.
    
    \item The agent $\agent$ visits each (environment)-state action pair infinitely often.
    
    %\item The agent acts greedily according to $Q_t$ as $t \ra \infty$.
\end{enumerate}

Recall that under the above conditions, \citet{watkins1992q} prove that 
\begin{equation}
\label{proof_eq:lim_q_t}
\lim_{t\ra \infty} Q_t(o,a) = Q^*(o,a),\ \forall_{o,a \in \observations \times \actions}.
\end{equation}
By consequence, we know that for any choice of $\varepsilon \in \mathbb{R}_{> 0}$, there exists a time $t$ such that
\begin{equation}
\label{proof_eq:q_t_bounded}
    |Q_t(o,a) - Q^*(o,a)| \leq \varepsilon
\end{equation}
for every $(o,a)$ pair.

We know that the agent will act according to the greedy policy
\[
\pi_t(o_t) = \argmax_{a \in \actions} Q_t(o_t, a).
\]

Note that by \cref{proof_eq:q_t_bounded}, we know that the action chosen $a_t = \pi_t(o_t)$ is at most $2\varepsilon$ below optimal. Hence, the agent will act according to actions that are $2\varepsilon$ sub-optimal, and therefore setting $\epsilon = \frac{2\varepsilon}{1-\gamma}$ ensures the agent is performance bounded in the sense of \cref{def:distortion_time_t}. Note that for any desired threshold $\epsilon > 0$, we can adjust the $t$ to yield a tighter $\varepsilon$ to still satisfy the desired bound. Therefore, we ensure that eventually there exists a $t$ such that $\delta_t(\agent, \environment) \leq \epsilon$, for any $\epsilon > 0$. \qedhere
%Hence, for any choice of $\epsilon > 0$, by consequence of \cref{proof_eq:q_t_bounded} we know that the action
\end{dproof}
